Synthesizing Reactive Systems from Hyperproperties

We study the reactive synthesis problem for hyperproperties given as formulas of the temporal logic HyperLTL. Hyperproperties generalize trace properties, i.e., sets of traces, to sets of sets of traces. Typical examples are information-flow policies like noninterference, which stipulate that no sensitive data must leak into the public domain. Such properties cannot be expressed in standard linear or branching-time temporal logics like LTL, CTL, or CTL$^*$. We show that, while the synthesis problem is undecidable for full HyperLTL, it remains decidable for the $\exists^*$, $\exists^*\forall^1$, and the $\mathit{linear}\;\forall^*$ fragments. Beyond these fragments, the synthesis problem immediately becomes undecidable. For universal HyperLTL, we present a semi-decision procedure that constructs implementations and counterexamples up to a given bound. We report encouraging experimental results obtained with a prototype implementation on example specifications with hyperproperties like symmetric responses, secrecy, and information-flow.

==> NtoNminus1.tex <==
\section{$∀^n↦∀^{n-1}$ Reduction}


We can generalize Theorem~\ref{Nto1} as follows. Sometimes, the reduction to a single ∀ quantifier is impossible although it is possible to reduce the quantifier amount. Here we see a procedure to reduce the quantifier amount by one. We can do this iteratively until we find the minimal amount of quantifiers.

Let $φ = ∀π_1,π_2,\dots,π_n.\ φ'$ be a formula in $∀^n$.

\begin{definition}
	Define the 1-reduced formula of φ by
	$$ reduce_1(φ) \coloneqq ∀π_1,\dots,π_{n-1}.\ \bigwedge_{i∈1\dots n}\bigwedge_{j∈1\dots i-1}{φ'[π_i↦π_j][π_n↦π_i]} $$
\end{definition}

The intuition behind this is that in a formula with one path quantifier less, always two paths have to be identical. And for that, all possible $O(n^2)$ combinations have to be covered with conjunctions.

\begin{theorem}
	It holds that $φ\equiv reduce_1(φ)$ or $\nexists ϕ∈∀^{n-1}.\ ϕ\equiv φ$
\end{theorem}

\begin{proof}
	Suppose there is some $ϕ∈∀^{n-1}$ with $ϕ\equiv φ$. Now, we will prove that $ϕ \equiv reduce_1(φ)$. Let $S$ be an arbitrary set of traces. Let $S'=\{s\|s\<S, |s|\leq n-1\}$. Because $ϕ∈∀^{n-1}$ and therefore the $n-1$ path variables of ϕ can only talk over $n-1$ paths, $S \models ϕ$ is equivalent to $∀ s'∈S'.\ s'\models ϕ$, what is by assumption equivalent to $∀ s'∈S'.\ s'\models φ$. Now, φ operates on trace sets of only $n-1$ traces what means that at least two path variables of φ have to refer to the same trace. We would now like to prove that $s'\models φ ⇔ s'\models reduce_1(φ)$ for any $s'∈S'$.
	
	\begin{enumerate}
		\item["⇒":] $s'\models φ$ implies $s'\models φ[π_i↦π_j]$ for arbitrary $i$ and $j$ because $[π_i↦π_j]$ is equivalent to restricting $π_i$ and $π_j$ to be the same. Therefore, $s'\models φ$ implies $s'\models reduce_1(φ)$.
		\item["⇐":] Because there are only $n-1$ traces in $s'$, it is always the case that two path variables $π_i$ and $π_j$ with w.l.o.g. $i>j$ refer to the same trace. This behavior is encoded in the rewriting of $[π_i↦π_j]$. Writing $φ[π_i↦π_j][π_n↦π_i]$ is equivalent to enforcing $π_i$ and $π_j$ to be the same. ($[π_n↦π_i]$ is needed because we do no longer have the variable $π_n$ and need to use the (now) unused variable $π_i$). If all these rewritings hold on $s'$ at the same time, φ holds on $s'$.
	\end{enumerate}
	
	\noindent And $∀ s'∈S'.\ s'\models reduce_1(φ)$ is again equivalent to $S \models reduce_1(φ)$ because $reduce_1(φ)$ only reasons over $n-1$ traces.
	%\begin{flalign*}
	%&\ S\models ϕ\\
	%⇔ &\text{ all subsets of $S$ of size smaller than $n$ satisfy } ϕ\\
	%&\hspace{1cm}\text{(because ϕ cannot talk about more than $n-1$ traces)}\\
	%⇔ &\text{ all }s'∈S'\text{ satisfy }ϕ\\
	%⇔ &\text{ all }s'∈S'\text{ satisfy φ (by assumption }ϕ\equiv φ\text{)}\\
	%⇔ &\text{ all }s'∈S'\text{ satisfy }reduce_1(φ)\\
	%&\hspace{1cm}\text{(because no matter to which trace $π_n$ is assigned to, the formula holds)}\\
	%⇔ &\text{ all subsets of $S$ of size smaller than $n$ satisfy } reduce_1(φ)\\
	%⇔&\ S\models reduce_1(φ)
	%\end{flalign*}
	Because $ϕ\equiv reduce_1(φ)$ and $ϕ\equiv φ$ it holds that $φ\equiv reduce_1(φ)$.
\end{proof}

==> pcp.tex <==
\section{Proof of Theorem~\ref{pcp}}

In Post's Correspondence Problem (PCP)~\cite{post1946variant}, we are given two lists $\alpha$ and $\beta$ consisting of finite words from some alphabet $\Sigma$.
For example, $\alpha$, with $\alpha_1 = a$, $\alpha_2 = ab$ and $\alpha_3 = bba$ and $\beta$, with $\beta_1 = baa$, $\beta_2 = aa$ and $\beta_3 = bb$, where $\alpha_i$ denotes the $i$\emph{th} element of the list, and $\alpha_{i_j}$ denotes the $j$\emph{th} symbol of the $i$\emph{th} element.
In this example, $\alpha_{3_1}$ corresponds to $b$.
PCP is the problem to find an index sequence $(i_k)_{1 \leq k \leq K}$ with $K \geq 1$ and $1 \leq i_k \leq n$ for all $k$, such that $\alpha_{i_1}\dots\alpha_{i_K}=\beta_{i_1}\dots\beta_{i_K}$.
We denote the finite words of a PCP solution with $i_\alpha$ and $i_\beta$, respectively.
It is a useful intuition to think of the PCP instance as a set of $n$ domino stones.
%The first stone of our example is \stone{a}{baa}, the second is \stone{ab}{aa} and the third, and last, is \stone{bba}{bb}.
%Those stones must be arranged (where copying is allowed) to construct the same word with the $\alpha$- and $\beta$-concatenations.
A possible solution for this PCP instance would be $(3,2,3,1)$, since this stone sequence produce the same word, i.e., $bbaabbbaa = i_\alpha = i_\beta$.

Let a PCP instance with $\Sigma = \{a_1,a_2,..., a_n\}$ and two lists $\alpha$ and $\beta$ be given.
%We denote the $i$th element of a list with $\alpha_i$ or $\beta_i$ respectively.
We choose our set of atomic propositions as follows: $\mathit{AP} := I\;\dot \cup\;O$ with $I := \{i\}$  and $O:= (\Sigma \cup \{\dot a_1, \dot a_2,... ,\dot a_n\} \cup {\#})^2$, where we use the dot symbol to encode that a stone starts at this position of the trace. We write $\tilde{a}$ if we do not care if this symbol is an $a$ or $\dot{a}$ and use $*$ as syntactic sugar for an arbitrary symbol of the alphabet.

We encode the PCP instance into a HyperLTL formula that is realizable if and only if the PCP instance has a solution as follows:
\begin{align*}
\varphi_\mathit{reduc} := \forall \pi \exists \pi'.\;\varphi_\mathit{rel}(\pi) \rightarrow &\varphi_\mathit{is++}(\pi,\pi')\\
&{} \wedge \varphi_\mathit{start}(\varphi_\mathit{stone\&shift}(\pi,\pi'),\pi) \wedge \varphi_\mathit{sol}(\pi')
\end{align*}

\begin{itemize}
	\item  $\varphi_\mathit{rel}(\pi) := \neg i \U \G i$. This defines the set of \emph{relevant} traces trough our strategy tree.
	
	\item $\varphi_\mathit{is++}(\pi,\pi') := (\neg i_\pi \wedge \neg i_{\pi'} \U \G i_\pi \wedge \neg i_{\pi'} \wedge \X \G i_{\pi'}$. This defines that a trace $\pi'$ is a successor of $\pi$:
	
	\item $\varphi_{\text{sol}}(\pi) \coloneqq \G i_{\pi} \rightarrow (\bigvee_{i=1}^n(\dot a_i, \dot a_i)_{\pi}) \wedge (\bigvee_{i=1}^n (\tilde{a_i},\tilde{a_i})_{\pi}) \U \G (\#,\#)_{\pi}$. This ensures that there exists a ``solution'' trace, which encodes the solution sequence.
	
	\item $\varphi_\mathit{stone\&shift}(π,π')$ encodes a stone of the PCP instance and that for every sequence of stones $\pi$, exists a (possibly empty) sequence of stones $\pi'$ with the first stone cut off. It also asserts that the sequence on $π'$ is identical to the sequence on π with the first stone removed and one step shifted as the new relevant trace on $π'$ starts one step later. See~\cite{conf/concur/FinkbeinerH16} for details.
	
	\item $\varphi_\mathit{start}(\varphi,\pi):= \neg i_\mathit{\pi} \U \varphi \wedge \G i_\pi$ cuts off an irrelevant prefix until $\varphi$ starts.
	
	\item We furthermore assume that only singletons are allowed what can be achieved by a disjunction for each pair of atomic propositions. See~\cite{conf/concur/FinkbeinerH16}.
%	\item $\varphi_\mathit{shift}(\pi,\pi')$ encodes that for every sequence of stones $\pi$, exists a (possibly empty) sequence of stones $\pi'$ with the first stone cut off.
	
	%\item $\varphi_\mathit{term} := \F \G (\#,\#)_\pi$ denotes that every sequence of stones has to terminate with $(\#,\#)$.
\end{itemize}

Correctness follows from the exact same arguments as in~\cite{conf/concur/FinkbeinerH16}.
